CraftRTL: High-quality Synthetic Data Generation for Verilog Code Models with Correct-by-Construction Non-Textual Representations and Targeted Code Repair

Despite the significant progress made in code generation with large language models, challenges persist, especially with hardware description languages such as Verilog. This paper first presents an analysis of fine-tuned LLMs on Verilog coding, with synthetic data from prior methods. We identify two main issues: difficulties in handling non-textual representations (Karnaugh maps, state-transition diagrams and waveforms) and significant variability during training with models randomly making "minor" mistakes. To address these limitations, we enhance data curation by creating correct-by-construction data targeting non-textual representations. Additionally, we introduce an automated framework that generates error reports from various model checkpoints and injects these errors into open-source code to create targeted code repair data. Our fine-tuned Starcoder2-15B outperforms prior state-of-the-art results by 3.8%, 10.9%, 6.6% for pass@1 on VerilogEval-Machine, VerilogEval-Human, and RTLLM.

==> Table/ablation-multistage.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Ablation studies on Iterative Targeted Code Repair}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|cccccc|cc|}
\hline
\multirow{3}{*}{Model}  & \multicolumn{6}{c|}{VerilogEval} & \multicolumn{2}{c|}{RTLLM v1.1} \\ \cline{2-9} 
 & \multicolumn{3}{c|}{Machine (\%)} & \multicolumn{3}{c|}{Human (\%)} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Syntax (\%)\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Func. (\%)\end{tabular}} \\ \cline{2-7}
 & pass@1 & pass@5 & \multicolumn{1}{c|}{pass@10} & pass@1 & pass@5 & pass@10 & \multicolumn{1}{c|}{} &  \\ \hline
 SDG-CC & \textbf{78.1} & 86.0 & \multicolumn{1}{c|}{88.5} & 45.2 & 59.5 & 63.8 & \multicolumn{1}{c|}{93.1} & 62.1 \\
 SDG-CC-repair 1 & 77.9 & \textbf{88.6} & \multicolumn{1}{c|}{\textbf{90.7}} & 52.7 & 62.5 & 67.3 & \multicolumn{1}{c|}{89.7} & 55.2 \\
 SDG-CC-repair 2 & 77.6 & 88.2 & \multicolumn{1}{c|}{\textbf{90.7}} & \textbf{53.2} & \textbf{65.1} & \textbf{68.5} & \multicolumn{1}{c|}{93.1} & 55.2 \\ \hline
\end{tabular}%
}
\label{tab:ablation_quality}
\end{table}

==> Table/ablation-quality.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Ablation studies on Targeted Code Repair Pipeline}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|cccccc|cc|}
\hline
\multirow{3}{*}{Model}  & \multicolumn{6}{c|}{VerilogEval} & \multicolumn{2}{c|}{RTLLM v1.1} \\ \cline{2-9} 
 & \multicolumn{3}{c|}{Machine (\%)} & \multicolumn{3}{c|}{Human (\%)} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Syntax (\%)\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Func. (\%)\end{tabular}} \\ \cline{2-7}
 & pass@1 & pass@5 & \multicolumn{1}{c|}{pass@10} & pass@1 & pass@5 & pass@10 & \multicolumn{1}{c|}{} &  \\ \hline
 SDG-CC-repair & \textbf{78.1} & 86.0 & \multicolumn{1}{c|}{88.5} & 45.2 & 59.5 & 63.8 & \multicolumn{1}{c|}{93.1} & 62.1 \\
 SDG-CC-repair w/o self-consistent & 77.9 & \textbf{88.6} & \multicolumn{1}{c|}{\textbf{90.7}} & 52.7 & 62.5 & 67.3 & \multicolumn{1}{c|}{89.7} & 55.2 \\
 SDG-CC-repair w/o error report & 77.6 & 88.2 & \multicolumn{1}{c|}{\textbf{90.7}} & \textbf{53.2} & \textbf{65.1} & \textbf{68.5} & \multicolumn{1}{c|}{93.1} & 55.2 \\
 SDG-CC w/o & 77.6 & 88.2 & \multicolumn{1}{c|}{\textbf{90.7}} & \textbf{53.2} & \textbf{65.1} & \textbf{68.5} & \multicolumn{1}{c|}{93.1} & 55.2 \\ \hline
\end{tabular}%
}
\label{tab:ablation_quality}
\end{table}






==> Table/main_old.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Comparison of our  models against various baseline models. Some data are missing due to the models being close-sourced and the data not being reported previously. The \textbf{best} results are highlighted in bold. In VerilogEval,  outperforms all previous methods across all metrics, relatively surpassing previous open-source SOTA BetterV by 14.4\% and GPT-4 by 22.1\% on average. In RTLLM,  relatively surpasses previous open-source SOTA RTLCoder by 11.3\%.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|cccccc|cc|}
\hline
\multirow{3}{*}{Type} & \multirow{3}{*}{Model} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Open\\ source\end{tabular}} & \multicolumn{6}{c|}{VerilogEval} & \multicolumn{2}{c|}{RTLLM v1.1} \\ \cline{4-11} 
 &  &  & \multicolumn{3}{c|}{Machine (\%)} & \multicolumn{3}{c|}{Human (\%)} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Syntax (\%)\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Func. (\%)\end{tabular}} \\ \cline{4-9}
 &  &  & pass@1 & pass@5 & \multicolumn{1}{c|}{pass@10} & pass@1 & pass@5 & pass@10 & \multicolumn{1}{c|}{} &  \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Foundation\\ models\end{tabular}} & GPT-3.5 & \Circle & 46.7 & 69.1 & \multicolumn{1}{c|}{74.1} & 26.7 & 45.8 & 51.7 & \multicolumn{1}{c|}{89.7} & 37.9 \\
 & GPT4 & \Circle & 60.0 & 70.6 & \multicolumn{1}{c|}{73.5} & 43.5 & 55.8 & 58.9 & \multicolumn{1}{c|}{\textbf{100.0}} & \textbf{65.5} \\
 & Starcoder & \CIRCLE & 46.8 & 54.5 & \multicolumn{1}{c|}{59.6} & 18.1 & 26.1 & 30.4 & \multicolumn{1}{c|}{93.1} & 27.6 \\
 & CodeLlama & \CIRCLE & 43.1 & 47.1 & \multicolumn{1}{c|}{47.7} & 18.2 & 22.7 & 24.3 & \multicolumn{1}{c|}{86.2} & 31.0 \\
 & DeepSeek-Coder & \CIRCLE & 52.2 & 55.4 & \multicolumn{1}{c|}{56.8} & 30.2 & 33.9 & 34.9 & \multicolumn{1}{c|}{93.1} & 44.8 \\
 & CodeQwen & \CIRCLE & 46.5 & 54.9 & \multicolumn{1}{c|}{56.4} & 22.5 & 26.1 & 28.0 & \multicolumn{1}{c|}{86.2} & 41.4 \\ \hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}IT\\ baselines\end{tabular}} & ChipNeMo & \Circle & 43.4 & - & \multicolumn{1}{c|}{-} & 22.4 & - & - & \multicolumn{1}{c|}{-} & - \\
 & Thakur et al. & \CIRCLE & 44.0 & 52.6 & \multicolumn{1}{c|}{59.2} & 30.3 & 43.9 & 49.6 & \multicolumn{1}{c|}{86.2} & 24.1 \\
 & RTLCoder-Mistral & \CIRCLE & 62.5 & 72.2 & \multicolumn{1}{c|}{76.6} & 36.7 & 45.5 & 49.2 & \multicolumn{1}{c|}{96.6} & 48.3 \\
 & RTLCoder-DeepSeek & \CIRCLE & 61.2 & 76.5 & \multicolumn{1}{c|}{81.8} & 41.6 & 50.1 & 53.4 & \multicolumn{1}{c|}{93.1} & 48.3 \\
 & BetterV-CodeLlama & \Circle & 64.2 & 75.4 & \multicolumn{1}{c|}{79.1} & 40.9 & 50.0 & 53.3 & \multicolumn{1}{c|}{-} & - \\
 & BetterV-DeepSeek & \Circle & 67.8 & 79.1 & \multicolumn{1}{c|}{84.0} & 45.9 & 53.3 & 57.6 & \multicolumn{1}{c|}{-} & - \\
 & BetterV-CodeQwen & \Circle & 68.1 & 79.4 & \multicolumn{1}{c|}{84.5} & 46.1 & 53.7 & 58.2 & \multicolumn{1}{c|}{-} & - \\ \hline
\multirow{3}{*}{CodeV} & CodeV-CodeLlama & \CIRCLE & \textbf{78.1} & 86.0 & \multicolumn{1}{c|}{88.5} & 45.2 & 59.5 & 63.8 & \multicolumn{1}{c|}{93.1} & 62.1 \\
 & CodeV-DeepSeek & \CIRCLE & 77.9 & \textbf{88.6} & \multicolumn{1}{c|}{\textbf{90.7}} & 52.7 & 62.5 & 67.3 & \multicolumn{1}{c|}{89.7} & 55.2 \\
 & CodeV-CodeQwen & \CIRCLE & 77.6 & 88.2 & \multicolumn{1}{c|}{\textbf{90.7}} & \textbf{53.2} & \textbf{65.1} & \textbf{68.5} & \multicolumn{1}{c|}{93.1} & 55.2 \\ \hline
\end{tabular}%
}
\label{tab:main_exp}
\end{table}

==> Table/stacked_figure.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.46\textwidth}
\centering
        % Stack the table and figure
\captionsetup{type=table} 
\captionof{table}{Data quantity CC.}
\vspace{-0.1in}
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
\multicolumn{1}{c|}{Method}                                & \multicolumn{1}{c}{Quantity}                   \\ \midrule
\multicolumn{1}{c|}{KMap} & \multicolumn{1}{c}{12.5k} \\ \midrule
\multicolumn{1}{c|}{FSM}  & \multicolumn{1}{c}{8.0k} \\ \midrule
\multicolumn{1}{c|}{Waveforms} & \multicolumn{1}{c}{8.0k} \\ \midrule \midrule
\multicolumn{1}{c|}{CC Total}                                & \multicolumn{1}{c}{28.5k}                      \\ \bottomrule
\end{tabular}}
\label{table:cc}

%\vspace{0.1in}
    \includegraphics[width=1.1\textwidth]{Figs/fsm_output.pdf} % Replace with your image file
    \vspace{-0.4in}
    \captionof{figure}{State transition logic.}
    \label{fig:fsm_ouput}
    \end{minipage}\hfill
    % Algorithm block on the right
    \begin{minipage}{0.54\textwidth}
    % Algorithm block on the right
 \begin{algorithm}[H]
        \caption{Generate transition graph for Moore FSM.}
        \begin{algorithmic}
        
    \STATE \textbf{Input:} Number of states $n$, bit width of input $w$
    \STATE \textbf{Output:} FSM graph with transitions and states

    \STATE Initialize the number of states $n$ and bit width of input $w$
    \STATE Randomly generate a tree with $n$ nodes
    \STATE Define the root of the tree as the reset state
    
    \FOR{each node in the tree}
        \STATE Assign a unique state to the node
        \STATE Assign an output to the node
    \ENDFOR
    
    \FOR{each node in the tree}
        \STATE Add additional transition edges to form a graph
        \STATE Ensure that each node has an out-degree of $2^w$
    \ENDFOR
        \end{algorithmic}
     \label{alg:fsm}
      \end{algorithm}
    \end{minipage}
\end{figure}

==> prompts/code_repair_example.tex <==
\begin{tcolorbox}[width=1.0\linewidth, halign=left, colframe=black, colback=white, boxsep=0.01mm, arc=1.5mm, left=2mm, right=2mm, boxrule=1pt]
\footnotesize{
\vspace{5pt}
Your goal is to create an error-fixing Verilog practice problem for programmers. You will demonstrate a type of error that is commonly made by programmers.
Create an error repair practice problem with three components:
1. Problem description\\
2. Erroneous implementation\\
3. Hints for fixing\\

\vspace{5pt}
Here is an example:\\
\vspace{5pt}
<EXAMPLE>\\
The following Verilog module is intended to implement the specification below. However, there is a bug in the code which causes incorrect results. Please fix the bug to make the module work as intended.\\
\vspace{5pt}
Erroneous Implementation:\\
\vspace{5pt}
\begin{lstlisting}[language=verilog]
// Verilog code with the injected error
module example_module (
    input wire clk,
    input wire reset,
    output reg [3:0] counter
);

// Intended functionality:
// This module should count from 0 to 15 and then wrap around.

always @(posedge clk or posedge reset) begin
    if (reset) begin
        counter <= 4'b0000;
    end else begin
        counter <= counter + 1'b1; // Error injected: Should be 4'b1
    end
end

endmodule
\end{lstlisting}
Hints for Fixing:\\
1. Verify the bit-width of the counter and the increment operation.\\
2. Check the initialization and wrapping condition of the counter.\\
3. Ensure that the addition operation correctly handles the 4-bit counter.\\
\vspace{5pt}
</EXAMPLE>
\vspace{5pt}

Now, here is the commonly made error:\\
\vspace{5pt}
\texttt{`}\texttt{`}\texttt{`} \\
\textcolor{red}{\{error report\}} \\
\texttt{`}\texttt{`}\texttt{`}  \\
\vspace{5pt}
Inject the above error into the following module and create an error repair practice problem.\\
\vspace{5pt}
\texttt{`}\texttt{`}\texttt{`} \\
\textcolor{red}{\{code snippet\}} \\
\texttt{`}\texttt{`}\texttt{`}  \\


\vspace{5pt}
Output: 
}
\end{tcolorbox}
\noindent\begin{minipage}{\textwidth}
\captionof{figure}{Error report example for task_id vector3.}
\end{minipage}




\begin{tcolorbox}[width=1.0\linewidth, halign=left, colframe=black, colback=white, boxsep=0.01mm, arc=1.5mm, left=2mm, right=2mm, boxrule=1pt]
\footnotesize{
\vspace{5pt}
Your goal is to create an error-fixing Verilog practice problem for programmers. You will demonstrate a type of error that is commonly made by programmers.
Create an error repair practice problem with three components:
1. Problem description\\
2. Erroneous implementation\\
3. Hints for fixing\\

\vspace{5pt}
Here is an example:\\
\vspace{5pt}
<EXAMPLE>\\
The following Verilog module is intended to implement the specification below. However, there is a bug in the code which causes incorrect results. Please fix the bug to make the module work as intended.\\
\vspace{5pt}
Erroneous Implementation:\\
\vspace{5pt}
\begin{lstlisting}[language=verilog]
// Verilog code with the injected error
module example_module (
    input wire clk,
    input wire reset,
    output reg [3:0] counter
);

// Intended functionality:
// This module should count from 0 to 15 and then wrap around.

always @(posedge clk or posedge reset) begin
    if (reset) begin
        counter <= 4'b0000;
    end else begin
        counter <= counter + 1'b1; // Error injected: Should be 4'b1
    end
end

endmodule
\end{lstlisting}
Hints for Fixing:\\
1. Verify the bit-width of the counter and the increment operation.\\
2. Check the initialization and wrapping condition of the counter.\\
3. Ensure that the addition operation correctly handles the 4-bit counter.\\
\vspace{5pt}
</EXAMPLE>
\vspace{5pt}

Now, here is the commonly made error:\\
\vspace{5pt}
\texttt{`}\texttt{`}\texttt{`} \\
\textcolor{red}{\{error report\}} \\
\texttt{`}\texttt{`}\texttt{`}  \\
\vspace{5pt}
Inject the above error into the following module and create an error repair practice problem.\\
\vspace{5pt}
\texttt{`}\texttt{`}\texttt{`} \\
\textcolor{red}{\{code snippet\}} \\
\texttt{`}\texttt{`}\texttt{`}  \\


\vspace{5pt}
Output: 
}
\end{tcolorbox}
\noindent\begin{minipage}{\textwidth}
\captionof{figure}{Error report example for task_id vector3.}
\end{minipage}



